AILS-NTUA at SemEval-2025 Task 3: Leveraging Large Language Models and Translation Strategies for Multilingual Hallucination Detection

Multilingual hallucination detection stands as an underexplored challenge, which the Mu-SHROOM shared task seeks to address. In this work, we propose an efficient, training-free LLM prompting strategy that enhances detection by translating multilingual text spans into English. Our approach achieves competitive rankings across multiple languages, securing two first positions in low-resource languages. The consistency of our results highlights the effectiveness of our translation strategy for hallucination detection, demonstrating its applicability regardless of the source language.

==> tables/translation_comparison_iou.tex <==

\begin{table*}[ht!]
    \centering \small
    \renewcommand{\arraystretch}{0.5}
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l|c|c|c|c}
        \hline

       \multirow{2}{*}{\textbf{Language (id)}} & \multicolumn{2}{c|}{\textbf{Original Input-Output Pairs}} & \multicolumn{2}{c}{\textbf{Translated Input-Output Pairs}} \\ 
       
        & \textbf{No Translation} & \textbf{External Transl. - Original} & \textbf{LLM Translator} & \textbf{External Transl. - English} \\ \hline
        
        Arabic (ar)   & 0.470 & 0.317 & 0.510 & \textbf{0.584} \\
        
        Catalan (ca)  & 0.458 & 0.503 & 0.490 & \textbf{0.703} \\
        
        Czech (cs)    & 0.387 & 0.367 & 0.419 & \textbf{0.587} \\
        
        German (de)   & 0.500 & 0.472 & 0.480 & \textbf{0.587} \\
        
        English (en)  & 0.550 & \textbf{0.555} & -     & -     \\
        
        Spanish (es)  & 0.490 & 0.312 & 0.420 & \textbf{0.500} \\
        
        Basque (eu)   & 0.355 & 0.339 & 0.375 & \textbf{0.571} \\
        
        Farsi (fa)    & 0.501 & 0.498 & 0.523 & \textbf{0.754} \\
        
        Finnish (fi)  & 0.540 & -     & 0.530 & \textbf{0.683} \\
        
        French (fr)   & 0.490 & 0.430 & 0.450 & \textbf{0.617} \\
        
        Hindi (hi)    & 0.650 & 0.660 & 0.700 & \textbf{0.726} \\
        
        Italian (it)  & 0.620 & 0.604 & 0.730 & \textbf{0.802} \\
        
        Swedish (sv)  & 0.530 & -     & 0.570 & \textbf{0.601} \\
        
        Chinese (zh)  & 0.343 & 0.399 & 0.379 & \textbf{0.419} \\
        \hline
    \end{tabular}
        \caption{Translation Performance Comparison - IoU. The best-performing method per language is in \textbf{bold}.}
    \label{tab:translation_comparison_iou}
\end{table*}

